Statistical Location and Rotation-Aware Beam Search for Millimeter-Wave Networks

Beam training in dynamic millimeter-wave (mm-wave) networks with mobile devices is highly challenging as devices must scan a large angular domain to maintain alignment of their directional antennas under mobility. Device rotation is particularly challenging, as a handheld device may rotate significantly over a very short period of time, causing it to lose the connection to the Access Point (AP) unless the rotation is accompanied by immediate beam realignment. We study how to maintain the link to a mm-wave AP under rotation and without any input from inertial sensors, exploiting the fact that mm-wave devices will typically be multi-band. We present a model that maps Time-of-Flight measurements to rotation and propose a method to infer the rotation speed of the mobile terminal using only measurements from sub-6 GHz WiFi. We also use the same sub-6 GHz WiFi system to reduce the angle error estimate for link establishment, exploiting the spatial geometry of the deployed APs and a statistical model that maps the user position's spatial distribution to an angle error distribution. We leverage these findings to introduce SLASH, a Statistical Location and rotation-Aware beam SearcH algorithm that adaptively narrows the sector search space and accelerates both link establishment and maintenance between mm-wave devices. We evaluate SLASH with experiments conducted indoors with a sub-6 GHz WiFi Time-of-Flight positioning system and a 60-GHz testbed. SLASH can increase the data rate by more than 41% for link establishment and 67% for link maintenance with respect to prior work.

==> sec/Rotation_old.tex <==

\begin{figure*}[t]
\centering
        \subfigure[Normalized power spectral density] 
{\includegraphics[width=0.95\columnwidth]{pics/FFT_8cases.eps}\label{fig:power_spectral_density}}
	%\hfill
	\subfigure[Study of the frequency $f_{1/2}$ 
]{\includegraphics[width=0.7\columnwidth]{pics/BarPlot_DiffAngSpeeds.eps}\label{fig:power_f12}}
	\caption{On the left: Normalized power spectral density as a function of the normalized frequency. On the right: bar plot 
of the frequency $f_{1/2}$ at which the normalized power is equal to $1/2$.}
\vspace{-2mm}
\end{figure*}


\section{From TOF ranging to rotation} \label{sec:rotation}

\note[Domenico]{old text and experiments. The study is ongoing. Add concept of spatial profiling while rotating and problem of 
packet loss study. ToF changes are due to constructive and destructive interference while syncing to the signal. Spatial aliasing 
if we don't sample sufficiently fast (but sampling rate to avoid spatial aliasing may depend on the specific antenna). add plot 
about antenna pattern? differentiate between different type of rotations and which 
one we handle here. We are not affected by dead reckoning problem as the absolute rotation is immediately fix after the new
beam training. Compare against error of magnetometer?}
The second challenge of our system is that the UE 
loses its orientation with respect to the AP as soon as the UE rotates relatively to the AP.
%Hence a Link Maintenance is required.

%As shown in the previous sections, our system can use the location of the user to dynamically select the best beams for Link 
%Establishment. However, as soon as the UE rotates relatively to the AP, the mm-wave transmitter 
%loses its relative orientation with respect to the receiver and a Link Maintenance is required.
%the  does not know where to point to beam towards the target device (or in general towards a given sector, according to the 
%analysis in Section~\ref{sec:angle_error_model}), as a positioning system does not provide the relative orientation of 
%the transmitter with respect to the target. This assumption was implicitly assumed in the previous section and we now 
We investigate 
how to handle this problem using only radio measurements and without the use of any inertial sensors.
%from the same 2.4 GHz ToF positioning system. 
The intuition behind our methodology is that a short series of ToF ranging measurements can provide not only the distance to the 
target UE,
%\footnote{In a general setup, the positioning system runs continuously, and thus there is always one link actively sending 
%Probes for ToF ranging.}, 
but also information about the relative rotation of the UE with respect to the AP. 
Radiation patterns of WiFi antennas are such that a rotating UE causes slight variations on the 
measured ToF dominant 
path. Such 
particular patterns become evident in a transformed domain, namely the frequency domain.
For this study, we consider different representative tests that can be classified as follows:


\noindent {\bf Test A}: We consider two static cases without rotation. The first one is representative of an ideal case without 
multipath and is obtained by connecting AP and UE via a coaxial cable. In the second one, AP and UE are positioned at a distance 
of 10 m from each other in an open space environment where, instead, multipath can occur.\\
\noindent {\bf Test B}:  We consider the UE moving with respect to the AP without any rotation. Specifically, in one test, 
we move the UE in a long corridor, starting from 1 m up to 60 m away from the AP, at a speed of approximately 1 m/s. In a second 
test, the UE is moved in the opposite direction, i.e., starting 60 m away up to 1 m of distance from the AP.\\
\noindent {\bf Test C}: We place the UE at 10 m of distance from the AP, in an open area where multipath can occur. The UE
is mounted on top of a Kobuki Turtlebot II robot running ROS (Robotic Operative System) in order to produce different rotation 
speeds, namely 0.03, 0.08, 0.35 and 0.7 rad/sec. 
We use custom python scripts to accurately control the multiple sensors and motors of the 
robot.%, executed on a USB-connected server, .% which allow us to emulate realistic user movements.
 
We use our legacy WiFi positioning system to perform the ToF measurements~(details are presented in Section~\ref{subsec:tof_pos}).
For each experiment, we gather ToF measurements and calculate the median of sequences of 50 samples. We compute 
the power 
spectral density $P(f)$, and then normalize it after DC removal. We show the results in Fig.~\ref{fig:power_spectral_density} as 
a function of the normalized frequency. First, for the experiment with the coaxial cable (figure on the top left), the spectrum 
is pure white noise. Also the experiment in the open space and without any rotation (figure on the top right) does not show 
any significant frequency component. Second, for the tests with mobility (the two figures in the second row), it can be observed 
that a dominant component appears at a very low frequency. 
%These tests are also very little affected by any spurious frequency 
%components as mobility brings spatial diversity and helps to cancel out any potential noise in the measurement.
Finally, for the experiments in rotation, the spectral analysis shows 
that the frequency of the dominant component increases with the speed of rotation. The slowest rotation can be easily 
distinguished from moving UE.

{\bf Inferring UE state and rotation speed.} We introduce a simple criterion to infer UE state that is robust to noise in the 
measurements. We integrate the normalized power spectral density and calculate the 
frequency at which the normalized power is equal to 1/2: $\sum_{f_0}^{f_{1/2}} \text{P}(f)=\frac{P_{tot}}{2}$,
where $f_0$ is the first frequency component after the DC component and $P_{tot}$ is the total power after DC removal.
We show the results of this study in Fig.~\ref{fig:power_f12}. We can observe a clear pattern in the frequency $f_{1/2}$ 
according to the UE state. In particular, the static cases (labeled as ``Cable'' and ``Static at 10 m'' in the figure) require a much larger $f_{1/2}$ as they do not have a dominant frequency component.
The opposite holds for the mobility cases. We can then define a heuristic hypothesis test based on the frequency $f_{1/2}$. Let us 
define the three hypothesis $H_0$, $H_1$ and $H_2$ as:
%$H_0$ :\text{``Static''};
%$H_1$ :\text{``Mobility''};
%$H_2$ :\text{``Rotation''}.
\begin{equation}
\nonumber
\begin{cases}
H_0 :\text{``Static''}\\
H_1 :\text{``Mobility''}\\
H_2 :\text{``Rotation''}\\
\end{cases}
\end{equation}



The test is as follows: accept $H_1$ if $ f_{1/2} < \alpha_1  $, accept $H_2$  if $\alpha_1 \le f_{1/2} \le \alpha_2 $,
stay with $H_0$ if $f_{1/2} > \alpha_2$. We fix $\alpha_2=0.2$ as the white noise will tend to have a spectrum without significant 
components. In order to fix the threshold $\alpha_1$,  we consider a maximum walking 
speed of $3$~m/s. Assuming this speed in the tests with mobility, we have 
$f_{1/2}=0.0033=\alpha_1$. 
From Fig.~\ref{fig:power_f12}, we can observe that the test with the slowest rotation 
of $0.03$~rad/s results in $f_{1/2}=0.012>\alpha_1$. 

%If the system accepts the hypothesis $H_2$, we consider
For the UE under rotation, we compute the Pearson correlation coefficient of the 
experimental set of $f_{1/2}$ with respect to the real rotation speeds. The result is a very high correlation of 0.973.
We then compute the linear regression of the experimental $f_{1/2}$ with respect to the real rotation speed and obtain an error 
of at most $8\cdot 10^{-3}$ degrees over a time span of $2$\,ms (maximum size of 802.11ad data frames). 

%In the next section, we will use this regression and error as input of our  beam search algorithm.

%Once the device is detected in rotation, we then seek for the highest spike in the power spectrum. We then plot the results in 
%{\edd add here power of rotation vs spike}, that shows a good linear correlation between the two variables.



